Convex Estimation of the $\alpha$-Confidence Reachable Sets of Systems with Parametric Uncertainty

Accurately modeling and verifying the correct operation of systems interacting in dynamic environments is challenging. By leveraging parametric uncertainty within the model description, one can relax the requirement to describe exactly the interactions with the environment; however, one must still guarantee that the model, despite uncertainty, behaves acceptably. This paper presents a convex optimization method to efficiently compute the set of configurations of a polynomial dynamical system that are able to safely reach a user defined target set despite parametric uncertainty in the model. Since planning in the presence of uncertainty can lead to undesirable conservatives, this paper computes those trajectories of the uncertain nonlinear systems which are $\alpha$-probable of reaching the desired configuration. The presented approach uses the notion of occupation measures to describe the evolution of trajectories of a nonlinear system with parametric uncertainty as a linear equation over measures whose supports coincide with the trajectories under investigation. This linear equation is approximated with vanishing conservatism using a hierarchy of semidefinite programs each of which is proven to compute an approximation to the set of initial conditions that are $\alpha$-probable of reaching the user defined target set safely in spite of uncertainty. The efficacy of this method is illustrated on four systems with parametric uncertainty.

==> sections/prob_conf.tex <==
\section{Problem formulation}
\label{sec:prob}
<<<<<<< .mine
In this section, we present a methodology to estimate the time limited $\alpha$-confidence backwards reachable set of dynamic systems. The proposed methodology consists of two steps -- (1) estimating the set of all feasible initial conditions of the system in Eqn.~(\ref{eq:aug_system}) such that $\gamma(T)\in X_T\times \Theta$; (2) determining the subset of initial conditions that reach the target set with desired probability. The first step is addressed by solving one of a pair of infinite dimensional problems, and the second step is performed on the optimal solution of Step (1).
\par
To estimate the BRS, we use the notion of {\em occupation measures} which was first introduced in \cite{Pitman1977}. Given an initial condition for the system, the occupation measure evaluates to the amount of time spent by the resultant trajectory in any subset of the space. The occupation measure $\mu(\cdot\mid x_0,\theta)\in \mathcal M_+(\mathcal T\times X\times \Theta\mid x_0,\theta)$ is formally defined as follows:
=======
In this section, we present a methodology to compute the time limited $\alpha$-confidence backwards reachable set of dynamic systems. The proposed methodology consists of two steps -- (1) estimating the set of all feasible initial conditions of the system in Eqn.~(\ref{eq:aug_system}) such that $\gamma(T)\in X_T\times \Theta$; (2) determining the subset of initial conditions that reach the target set with desired probability. The first step is addressed by solving an infinite dimensional problem, and the second step requires integrating the optimal solution of Step (1).

To estimate the BRS, we use the notion of {\em occupation measures} [Pitman]. Given an initial condition for the system, the occupation measure evaluates to the amount of time spent by the resultant trajectory in any subset of the space. The occupation measure $\mu(\cdot\mid x_0,\theta)\in \mathcal M_+(\mathcal T\times X\times \Theta\mid x_0,\theta)$ is formally defined as follows:
>>>>>>> .r67
\begin{align}
  \mu(A\times B\times C\mid x_0,\theta) = \int_{0}^T I_{A\times B\times C}(t,x,\theta\mid x_0,\theta)\,dt,
  \label{eq:occ}
\end{align}
where $I_{A}(\cdot)$ is the indicator function on the set $A$ that returns one if $x\in A$ and zero otherwise. With the above definition of the occupation measure, using elementary functions, it can be shown that:
\begin{align}
  \ip{\mu(\cdot\mid x_0,\theta),v} = \ip{\lambda_t,v(t,x(t\mid x_0,\theta),\theta)},
  \label{eq:ip}
\end{align}
where $\lambda_t$ is the Lebesgue measure on $\mathcal T$.

The {\em occupation measure} has an interesting characteristic -- it completely characterizes the solution trajectory of the system resulting from an initial condition. Observe that the occupation measure as defined in Eqn.~(\ref{eq:occ}) is conditioned on the initial values of states and parameters. Since we are interested in the collective behavior of possibly collection of initial conditions, we define the {\em average} occupation measure as:
\begin{align}
\mu(A\times B\times C) = \int_{X\times \Theta} \mu(A\times B\times C\mid x,\theta)\,d\mu_0,
\end{align}
where $\mu_0$ is the un-normalized distribution of the initial conditions. The value to which the {\em average} occupation measure evaluates over a given set in $\mathcal T\times X\times \Theta$ can be interpreted as the cumulative time spent by all solution trajectories which begin in $\spt(\mu_0)$.
\par
Given a test function $v\in \mathcal C^1(\mathcal T\times X\times \Theta)$, using the Fundamental Theorem of Calculus, its value at time $t=T$ is given by
\begin{align}
\begin{split}
  v(T,x(T\mid x_0,\theta),\theta) =&\, v(0,x_0,\theta)\\
  +&\,\int\limits_{0}^T\hspace*{-.08in}\left(\frac{\partial v}{\partial x}\cdot \tilde f+\frac{\partial v}{\partial t}\right)(t,x(t\mid x_0,\theta),\theta)\,dt
\end{split}
  \label{eq:ftc}
\end{align}
Using the relation defined in Eqn.~(\ref{eq:ip}) and by defining the linear operator $\mathcal L_f$ on $\mathcal C^1$ functions (Lie derivative) as the following:
\begin{align}
  \mathcal L_{\tilde f}v = \frac{\partial v}{\partial x}\cdot \tilde f+ \frac{\partial v}{\partial t},
\end{align}
Eqn.~(\ref{eq:ftc}) is re-written as
\begin{align}
\begin{split}
  v(T,x(T\mid x_0,\theta),\theta) =&\, v(0,x_0,\theta)\\
  +&\,\int\limits_{X\times \Theta}\mathcal L_{\tilde f}v\,d\mu(t,x,\theta\mid x_0,\theta).
\end{split}
\label{eq:ftc2}
\end{align}
Integrating Eqn.~(\ref{eq:ftc2}) with respect to $\mu_0$, the distribution of initial conditions, and defining a new measure $\mu_T\in \mathcal M_+ (X_T\times \Theta)$, as the following
\begin{align}
  \mu_T(A\times B) = \int\limits_{X\times \Theta}I_{A\times B}(x(T\mid x_0,\theta),\theta)\,d\mu_0,
\end{align}
produces the following equality
\begin{align}
  \ip{\delta_T\otimes \mu_T,v}= \ip{\delta_0\otimes \mu_0,v}+\ip{\mu,\mathcal L_{\tilde f}v},
  \label{eq:lv}
\end{align}
<<<<<<< .mine
where with a slight abuse of notations, $\delta_t$ is used to denoted a dirac measure situated at $t$. Equation~(\ref{eq:lv}) is a version of the Liouville equation, holds for all test function $v\in \mathcal C^1(\mathcal T\times X\times \Theta)$, and summarises the visitation information of all trajectories that emanate from $\spt(\mu_0)$ and terminate in $\spt(\mu_T)$. The interested reader to directed to \cite{henrion2014convex} to a more detailed discussion on the Liouivlle equation and the implication of the existence of measures that satisfy the same.
\par
=======
where with a slight abuse of notations, $\delta_t$ is used to denoted a dirac measure situated at $t$. Equation~(\ref{eq:lv}) is a version of the Liouville equation, holds for all test function $v\in \mathcal C^1(\mathcal T\times X\times \Theta)$, and summarises the visitation information of all trajectories that emanate from $\spt(\mu_0)$ and terminate in $\spt(\mu_T)$. Several recent papers provide a more detailed discussion on the Liouville equation [Henrion].

>>>>>>> .r67
Within this framework of measures and the Liouville Equation, we first formulate the problem of identifying the set of all pairs $(x_0,\theta)$ such that the solution trajectory of the system in Eqn.~(\ref{eq:aug_system}) initialized at $[x;\,\theta]$ arrives at $X_T\times \Theta$ at $t=T$. This problem can be interpreted as one that attempts to identify the largest support for $\mu_0$ such that there exist measures $\mu$ and $\mu_T$ such that $(\mu_0,\mu_T,\mu)$ satisfy Eqn.~(\ref{eq:lv}). To measure the size of $\spt(\mu_0)$, we use the Lebesgue measure on $X\times \Theta$, $\lambda_x\otimes \lambda_\theta$.
\par
This problem is posed as an infinite dimensional Linear Program (LP) on measures as defined below.
%
%To identify the $\alpha$-confidence
%
%can be formulated as the following infinite-dimensional linear program that supremizes the \emph{volume} of the set of initial pairs of $x$ and uncertain parameter, $\theta$, such that the state trajectories, at time $T$, arrive in $X_T$ :
\begin{flalign}\nonumber
    & & \sup_{\Lambda} \hspace*{1cm} & \ip{\mu_{0},\mathds 1} && (P)\\
    & & \text{st.} \hspace*{1cm} &\mu_{0}+\mathcal L_{f}'\mu=\,\mu_{T} && \label{eq:primal:liouville}\\
    & & & \mu_{0}+\hat\mu_{0}=\,\lambda_x\otimes \lambda_\theta &&
\end{flalign}
where $\lambda_x\times \lambda_\theta$ is the Lebesgue measure supported on $X\times \Theta$, $\Lambda:=(\mu_0,\hat\mu_{0},\mu_T),\in {\mathcal M}_+({\mathcal T} \times X \times \Theta) \times \mathcal M_+( X \times \Theta)\times \mathcal M_+( X_{T}\times \Theta )$, and $\mathds 1$ denotes the function that takes value $1$ everywhere.
\begin{lem}
  The support of $\mu_0$, $\spt(\mu_0)\subset X\times \Theta$ is the largest collection of pairs $(x,\theta)$ that, if used as initial conditions to Eqn. \eqref{eq:aug_system}, produce a solution trajectory that terminates in $X_T\times \Theta$ at $t=T$.
\end{lem}
\par
The dual problem, on continuous functions, corresponding to $(P)$ is the following
\begin{flalign}\nonumber
  & &  \inf_{\Xi}&\phantom{3} \ip{\lambda_x\otimes \lambda_\theta,w}          && (D) \nonumber \\
  & &  \text{st.}&\phantom{3}\mathcal L_{\tilde f} v(t,x,\theta)\le 0         && \forall (t,x,\theta)\in \mathcal T\times X\times\Theta\\
  & &  &\phantom{3} w(x,\theta) \ge 0                                         && \forall (x,\theta)\in X\times\Theta\\
  & &  &\phantom{3} w(x,\theta) - v(0,x,\theta) - 1 \ge 0                     && \forall (x,\theta)\in X\times\Theta\\
  & & & \phantom{3} v(T,x,\theta)\ge 0                                        && \forall (x,\theta)\in X_T\times \Theta
\end{flalign}
where $\Xi := (v,w)\in \mathcal C^1(\mathcal T\times X\times \Theta)\times \mathcal C(X\times \Theta)$. The solution to $(D)$ has an interesting interpretation: $v$ is similar to a Lyapunov function for the system, and $w$ resembles an indicator function on $\spt(\mu_0)$. Moreover:
\begin{lem}
  There is no duality gap between problems $(P)$ and $(D)$.
\end{lem}
\begin{lem}
  Given the pair of functions $(v^*,w^*)$ which is the optimal solution to $(D)$, the 1-super-level set of $w^*$ contains $\spt(\mu_0)$.
\end{lem}
The following salient result on the form of $w$ is a critical result that we will employ to estimate $X_0$ as defined in Defn.~\ref{defn:brs}.
\begin{thm}[henrion, thm 3]
\label{thm:indicator}
 There is a sequence of feasible points to $(D)$ whose $w$ component converges uniformly in the $L^1$ norm to the indicator function on $\spt(\mu_0)$.
\end{thm}
The immediate consequence of the above theorem is that we can assume that $w$ evaluates to one on $\spt(\mu_0)$ and zero elsewhere. Now, relating the definition of $\Gamma$ in Eqn.~(\ref{eq:Gamma}) and this feature of $w^*$, the $w$ component of the optimal solution of $(D)$, one arrives at the following result that provides a means to compute the $\alpha$-confidence time limited reachable set, $X_0$.
\begin{lem}
Suppose $(v^*,w^*)$ is an optimal solution of $(D)$. The $\alpha$-level backwards reachable of the set $X_T$ under the dynamics in Eqn.~(\ref{eq:aug_system}) and parametric uncertainty with distribution $\mu_\theta$ is given by the following set
\begin{align}
X_0^\alpha:=\bigg\{x\,\big \mid \int_\Theta w^*(x,\theta)\,d\mu_\theta\ge \alpha \bigg\}
\end{align}
\label{lem:confidence}
\end{lem}
\begin{proof}
%There exists a sequence $w_k$ of feasible $w$ in $(D)$ that converges to the indicator function $I_{\Gamma(x)}(x,\theta)$ in the $L^1$ norm (REFERENCE H-K PAPER). Therefore, the optimal solution $w^*$ is $I_{\Gamma(x)}(x,\theta)$. So, for any $x$,
%\begin{align}
%\int_\Theta w^*(x,\theta)\,d\mu_\theta &= \int_{\Gamma(x)} \mathds 1\,d\mu_\theta = \mu_\theta(\Gamma(x))
%\end{align}
Using the provided information, define the measure $\eta\in \mathcal M_+(X\times \Theta)$ as follows:
\begin{align}
  \eta(A\times B) = \int_{A\times B} w^*(x,\theta) \,d(\lambda_x\otimes \mu_\theta).
\end{align}
It should be noted that $\Gamma(x)$ as defined in Eqn.~(\ref{eq:Gamma}) is the support of the conditional distribution of $\theta$ given $x$ of $\eta$; $\spt(\eta(\cdot\mid x))$. This is true since for $w^*$ is an indicator function on $\spt(\mu_0)$, the set of all feasible pairs $(x,\theta)$.
In addition, by definition, $\lambda_x\otimes \mu_\theta \gg \eta$ and hence $\lambda_x\gg \pi^x_*\eta$, where $\pi^x_*$ is the push-forward of measure of $\eta$ under the projection operator \cite{lee2003smooth}. There exists $\phi(x)$ that is the Radon-Nikodym derivative between $\lambda_x$ and $\pi_*^{x}\eta$, the $x$-projection of $\eta$ such that
\begin{align}
  \pi^x_*\eta(A) =&\, \int_A \phi(x)\,d\lambda_x,\phantom{4}\forall A\subset X.
\end{align}
The function $\phi(x)$, for each $x$ evaluates to the probability that $x$ will reach $X_T$ given the distribution of uncertainty. To see this, observe that
\begin{align}
  \int_A \phi(x)\,d\lambda_x = &\,\int_A \int_\Theta w^*\,d\,\mu_\theta d\lambda_x,\\
  =&\, \int_A \int_{\Gamma(x)} w^*\,d\,\mu_\theta d\lambda_x,\\
  =&\, \int_A \int_{\Gamma(x)} 1\,d\,\mu_\theta d\lambda_x,
\end{align}
where we have used the fact that $w^*\ge 1,\, \forall(x,\theta)\in \spt(\mu_0)$ (from Thm.~\ref{thm:indicator}), that $\mu_\theta$ is a probability measure, and Defn.~\ref{defn:brs}. The statement of the Lemma now follows from Defn.~\ref{defn:brs}.
\end{proof}
Lemma~\ref{lem:confidence} provides a means to compute the $\alpha$-confidence $T$-time backwards reachable set; one just has to integrate the $w$ component of the optimal solution to $(D)$ with respect to the distribution of $\theta$ and identify level sets. Solving the infinite dimensional problem is nontrivial; in the following section, we employ Lasserre's hierarchy of relaxations to arrive at a sequence of outer approximations of $X_0^\alpha$.

